Video Action Differencing

How do two individuals differ when performing the same action? In this work, we introduce Video Action Differencing (VidDiff), the novel task of identifying subtle differences between videos of the same action, which has many applications, such as coaching and skill learning. To enable development on this new task, we first create VidDiffBench, a benchmark dataset containing 549 video pairs, with human annotations of 4,469 fine-grained action differences and 2,075 localization timestamps indicating where these differences occur. Our experiments demonstrate that VidDiffBench poses a significant challenge for state-of-the-art large multimodal models (LMMs), such as GPT-4o and Qwen2-VL. By analyzing failure cases of LMMs on VidDiffBench, we highlight two key challenges for this task: localizing relevant sub-actions over two videos and fine-grained frame comparison. To overcome these, we propose the VidDiff method, an agentic workflow that breaks the task into three stages: action difference proposal, keyframe localization, and frame differencing, each stage utilizing specialized foundation models. To encourage future research in this new task, we release the benchmark at https://huggingface.co/datasets/jmhb/VidDiffBench and code at http://jmhb0.github.io/viddiff.

==> sec/benchmark.tex <==
\section{Evaluation benchmark}
\label{sec:benchmark}
Our evaluation benchmark emphasizes comparing skilled video action differencing, since this is well-motivated by applications.
The zero-shot benchmark evaluates \textit{generalizability} to many action categories by including diverse in-the-wild video categories (\Cref{sec:task_and_benchmark-benchmark-videos}), and its annotations are \textit{relevant} to skills applications by utilizing expert knowledge (\Cref{sec:task_and_benchmark-benchmark-annotations}). The dataset categories and statistics are in \Cref{tab:benchmark summary}. In \Cref{sec:task_difficulty}, we characterize the key challenges for this task. This is illustrated in \Cref{fig:benchmark_difficulty}, and we use it to dataset splits in \Cref{tab:benchmark_challenges}.

\input{tables/benchmark_summary}

\subsection{Videos}
\label{sec:task_and_benchmark-benchmark-videos}

We first identified datasets in computer vision literature for video perception, action quality assessment, and action feedback across a diverse coverage of skilled activities in sports, music, and surgery. 
We had three criteria for benchmark videos. 
First, videos should be short and contain a single action, for example a basketball shot, but not a full volleyball rally \cite{li2021multisports} or a long gymnastics sequence \cite{shao2020finegym}. This is because motor skill training focuses on discrete motions of one actor. 
Second, we choose  actions with a consistent sequence of sub-actions, which excludes open-ended activities like rock climbing or salsa dancing \cite{grauman2023ego}. This is because the `fixed action transcript' assumption allows methods to exploit known task structure, and we believe the assumption still holds  for a very wide range of skills.
Third, most relevant differences should be simple, visual, and tangible; this excludes salsa dancing for example because feedback can include `looseness in the knees' or `good flow', which is challenging to visually characterize.

Since most datasets were untrimmed, we annotated the action's start and end frames.  
To support our motivation of video differencing for comparing novices to experts, we used data sources where user skill level variation was high \cite{parmar2022domain_fitnessaqa, grauman2023ego, gao2014jhu}, and we randomly sample videos to have a roughly equal proportion of skill levels (\Cref{sec:appendix-video_selection}).
We then randomly generate video pairs, and we remove videos that have fewer than 3 annotated differences.
% Datasets with skill-level annotation \cite{grauman2023ego}, action error annotation \cite{parmar2022domain_fitnessaqa}, and quality scores \cite{xu2022finediving} were especially useful.
% Additionally, for `ballsports; and `surgery' categories, we include video pairs that are the same action by the same user \cite{grauman2023ego}, since this is another motivating application (todo: stats for that). 
The videos are all in-the-wild (except for Fitness) and with varying camera perspective (except for Diving), which is realistic and challenging. 

% Exceptions were fitness where there is not variation in skill level, but we chose to include since they are simpler motions that are useful for easy benchmark; and Diving, were all motions are professionals, but we included it for a secondary application, which is AQA explainability.

% Another choice is what camera angle do we want? In EgoExo4D and for Hummann, we could choose it. In others we can't. BUT we can choose which
% What we could say is `look at the existing variations', and say what is the best angle to judge certain things. 
% For FineDiving, it's standardized, which is again realistic to applications. 


\subsection{Natural language difference annotations}
\label{sec:task_and_benchmark-benchmark-annotations}
For each action, we create a difference taxonomy, which is a list of differences that are relevant to performing that action, and are visually assessable. For example in basketball jump shot, one difference is ``ball more in front of the body''; then we annotate `A' if more true in video A, `B' if more true in video B, and `C' if it is similar or too hard to tell. 

\begin{figure}
  \centering
  % \fbox{\parbox[c][5cm][c]{5cm}{\centering Placeholder}} % creates a box with centered text "Placeholder"
  \includegraphics[width=\columnwidth]{figs/fig_challenges_may13.png}
  \caption{The three types of difficulty identified in our VidDiff benchmark. Top: for \textit{domain specificity}, specialized domains like surgery perform worse in all three stages of our framework, probably due to coverage in zero-shot models. Bottom left: for \textit{retrieval precision}, the correct retrieval identifies that `A' squats deeper, but a small error in retrieval frame can reverse the conclusion. Bottom right: for \textit{fine-grained difference}, the same action and difference question is harder if the difference is more fine-grained.
  }
  \label{fig:benchmark_difficulty}
\end{figure}


We use expert domain knowledge to define the taxonomy, which depends on the data source, and we give a fuller description in \Cref{sec:appendix_difference_taxonomy}. For Fitness and Surgery, we take sample videos from experts and novices, and ask a domain expert to propose a list of differences that are both relevant to the activity and also visible in the videos. For Ballsports and Music, we leverage the unstructured expert commentary annotations from Ego-Exo4D ~\cite{grauman2023ego}. Specifically, we feed the text strings to an LLM and ask it to summarize the  relevant visual differences (details in \Cref{sec:appendix_difference_taxonomy-egoExo4D_processing}). 
For Diving, we again utilize an LLM, this time to summarize the text from the guidebook for judging dive quality. 
For weightlifting, we leverage the error classes that are proposed in the source Fitness-AQA dataset ~\cite{parmar2022domain_fitnessaqa}. 

Given the proposed taxonomy, we then filter out differences that are not assessable in the videos. 
% Maybe a comment on 
For example in basketball jump shot, the difference ``elbow more tucked in'' is too difficult to assess from the given camera angles, and ``wrist snap gives more backspin'' is difficult because the ball spinning speed is not visible. 
The complete taxonomy is in ~\Cref{sec:appendix-the_difference_taxonomy}.

% TODO: maybe a comment on continuous vs binary differences.
A human annotator then manually inspects each video pair, and for each candidate difference from the taxonomy, chooses whether the statement more applies to `video A', `video B', or `neither'. Importantly, annotators are instructed only to choose `A' or `B' if they can clearly perceive the difference, and to choose `C' otherwise. \AR{TODO for Anita: We relabeled a sub-sample of pairs by a second annotator to ensure consistency...}

\subsection{Retrieval annotations}
\label{sec:benchmark-retrieval_annot}
Recall that in our method's final stage -- the frame differencer -- the input is candidate differences with the relevant frames identified by the retriever , which are then combined into an image QA query (\Cref{sec:methods-differencer}, \Cref{fig:method}). 
We provide human-generated annotations to identify relevant frames, which we detail in \Cref{sec:appendix-retrieval_annotations}. In evaluation, this enables isolating the accuracy of the frame-differencer. These annotations could form a part of evaluation benchmarks for general image understanding \cite{Fu2023MMEAC}, or for moment localization\cite{gu2018ava}.

\subsection{Difficulty levels and data splits}
\label{sec:task_difficulty}


We identify three axes of difficulty, illustrated in  \Cref{fig:benchmark_difficulty}. For \textit{domain specificity}, zero shot models have poor coverage of certain domains like surgery. This affects every aspect of our method: the LLM may not have the knowledge to propose good variations, predict the sub-action transcript, or give good retrieval strings; in retrieval, the CLIP model may have poor text-image alignment for the task; and the VLM in the frame differencer will perform poorly. \textit{Retrieval precision} applies to certain variations where a small retrieval error leads to an incorrect answer. For example in the bottom left box, to assess who has `deeper squat depth', we need the frame where the squatter is lowest, but an error of less than 0.1 seconds will lead to the wrong conclusion. \textit{Fine-grained differences} apply to the frame differencer: once the frames are retrieved, a VLM will perform worse with a lower-magnitude difference. 

We use this characterization to define difficulty splits, as shown in \Cref{tab:benchmark summary}. The easiest split scores low in all three; the medium split adds `fine-grained differences' since it is relevant to the final stage only; and the hard split is hard in all dimensions. Data with hard `domain spcificity' is chosen based on category: only surgery and diving are hard. Data with `high retrieval precision is chosen based on the difference taxonomy. For `very fine-grained differences', we choose a subset of variations where differences are clear, and we ask annotators to choose video pairs where the difference is large. 

\input{tables/benchmark_difficulty}



\subsection{Evaluation}
\label{sec:task_and_benchmark-evaluation}
In the standard (open) evaluation, the system outputs a list of text strings that are proposed differences which should correspond to the differences in the benchmark taxonomy. We utilize ChatGPT to propose a matching between the pairs; the prompt details are in \Cref{sec:appendix-eval_matching}.
For `closed evaluation' and post-retrieval evaluation, the benchmark's differences are provided, so this matching is not necessary. The metric is accuracy. 

% Metrics: precision and recall for differences. TODO: decide whether we want to punish choosing `c' when answer is `a' or `b' i.e. do we prefer the systems to be more conservative. 



